Lumos: Increasing Awareness of Analytic Behavior during Visual Data Analysis

Visual data analysis tools provide people with the agency and flexibility to explore data using a variety of interactive functionalities. However, this flexibility may introduce potential consequences in situations where users unknowingly overemphasize or underemphasize specific subsets of the data or attribute space they are analyzing. For example, users may overemphasize specific attributes and/or their values (e.g., Gender is always encoded on the X axis), underemphasize others (e.g., Religion is never encoded), ignore a subset of the data (e.g., older people are filtered out), etc. In response, we present Lumos, a visual data analysis tool that captures and shows the interaction history with data to increase awareness of such analytic behaviors. Using in-situ (at the place of interaction) and ex-situ (in an external view) visualization techniques, Lumos provides real-time feedback to users for them to reflect on their activities. For example, Lumos highlights datapoints that have been previously examined in the same visualization (in-situ) and also overlays them on the underlying data distribution (i.e., baseline distribution) in a separate visualization (ex-situ). Through a user study with 24 participants, we investigate how Lumos helps users' data exploration and decision-making processes. We found that Lumos increases users' awareness of visual data analysis practices in real-time, promoting reflection upon and acknowledgement of their intentions and potentially influencing subsequent interactions.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> src/sections/bias_metrics_review.tex <==
\arpit{for reference -- to be rewritten}

While several metrics have been proposed to quantify aspects of a user's analysis process (e.g.,~\cite{feng2019patterns,jankun2000spreadsheet,wall2017warning}), here we focus on bias metrics~\cite{wall2017warning} which are theoretically applicable to various types of bias and have been used for initial characterization of anchoring bias~\cite{wall2019formative}. 
We quantify bias using the following two metrics: data point distribution (DPD) and attribute distribution (AD)~\cite{wall2017warning}. 
These metrics characterize, along a scale from 0 (no bias) to 1 (high bias), how a user's interactive behavior deviates from expected behavior. 
In this case, expected behavior is defined by equal probability of interaction with any given data point in the dataset. \arpit{todo: equal and custom baselines are also there.}

Consider a dataset of movies. Data point distribution (DPD) describes how the user's interactions are distributed over the dataset. 
Uniform interactions over all movies will result in a low metric value (less biased), while repeated interaction with a subset of the data (e.g., only \attr{Action} movies) will result in a higher metric value (more biased).

Attribute distribution (AD) considers how the users' interactions across the data map to the underlying distributions of each attribute. That is, if the dataset has movies with an average \attr{Running Time} of 90 minutes, but the user focuses almost exclusively on longer movies (potentially revisiting the same subset of long movies), the attribute distribution metric for \attr{Running Time} would be high (more biased). 

Alternatively, if the user's interactions are proportional to the dataset, the metric value would be low (less biased). \arpit{modify this to include equal, custom stuff}

These metrics drive the visualization and study design in this paper that shows a user's interaction traces as they make their decisions.


==> src/sections/study-notes.tex <==
% Control
\subsubsection{CONTROL}
\bpstart{P09}
\begin{enumerate}[nosep]
    \item ++++ (how showing attribute interaction traces can be useful) -- ``Experimenter observed the participant count the attributes they had interacted with until then (speak + gesture by hand)''
    \item ---- (undo an accidental interaction trace?) -- ``I accidentally created this visualization.''
\end{enumerate}

\bpstart{P10}
\begin{enumerate}[nosep]
    \item ++++ (why black, data curves in the distribution panel can be useful) -- ``(by creating simple visualizations) I'm just trying to see what types of values/categories are there in the dataset''
    \item ++-- (weak signal to motivate the blue colorings) -- ``I really like things when there are colors in the interface''
\end{enumerate}

\bpstart{P11}
\begin{enumerate}[nosep]
    \item ++++ (why black, data curves in the distribution panel can be useful) -- ``(added filters to gauge the categories/values in the data for the attributes.)''
    \item ++-- (weak signal to motivate the blue colorings) -- ``I really like things when there are colors in the interface''
    \item ++++ (positive feedback) -- ``Prompts were nice; swap-axes feature was nice; filtering was nice;''
    \item ++++ (how showing attribute interaction traces can be useful) -- ``(while filling the post-study questionnaire to gauge individual focus on each attribute) I didn't consider this attribute at all now that I'm seeing this in the form.''
\end{enumerate}

\bpstart{P12}
\begin{enumerate}[nosep]
    \item ++++ (ticks in charts) -- ``I like the design of these ticks - one long one short''
    \item ++++ (feature request) -- ``I want to be able to derive attributes (e.g., Worldwide grosss / Production Budget)''
    \item ++++ (motivation for distribution panel) -- ``Participant created a strip plot of Creative Type to see the distribution of various categories''
    \item ++++ (feature request) -- ``One thing I notice is that if I switch attributes, I want to see which points moved where'' (add transitions)
    \item ---- (Details view (single point)) -- ``I didn't use the details view (single point) because my analysis was at a very low-level'
    \item ++++ (Details view (agg point)) -- ``Good to inspect raw data (in the bar) as now user doesn't need to open it in Excel or GSheets.''
\end{enumerate}

\bpstart{P16}
\begin{enumerate}[nosep]
    \item ++++ (general feedback) -- \emph{``I like the interface design, it’s very clean. As a user, if I’m doing data, it really helps to have a minimalist interface design''}
    \item ++++ (details view) -- \emph{``I really like the Details portion and being able to hover over points for more details.''}
    \item ++-- (filters) -- \emph{``I like (to) have Filters; however, having Filters reduces the overall ability to see the bigger picture.''}
    \item ++++ (attribute panel) -- \emph{``I found it very useful to have all of the Attributes listed out at all times, versus for example Excel where they aren’t always on-screen''}
    \item ++++ (nice point on aggregation details view) -- \emph{``It’s hard to draw conclusions from lists of words and data; I’d rather see the information visually''}
\end{enumerate}

\bpstart{P18}
\begin{enumerate}[nosep]
    \item ++-- (confound) -- \emph{``It is not apparent from the bar shape and size that some bars only have 1 points in them versus some bars having 6 or 7 points''}
    \item ++++ (motivation for distribution curves) -- \emph{``If I was in R, I could describe data variables by attribute -- meaning she would prefer getting the ranges, distributions, etc. of attribute values using R code.''}
    \item ++-- (personality, details view) -- \emph{``Details View was really useful because the Visualization Canvas wasn’t as helpful. I spent over half my time here!''}
\end{enumerate}

\bpstart{P19}
\begin{enumerate}[nosep]
    \item ++++ (control participant remembered this without blue colors) -- ``Ok so I haven’t looked at IMDB Rating at all yet...''
    \item ++-- (filters, motivation for distribution view) -- ``I think using Filters to see the distribution of values in an attribute is really great''
    \item ++++ (general) -- \emph{``When I saw the interface, it reminded me of Tableau!''}
    \item ---+ (details view unit) -- \emph{``I didn’t find the Details view for single datapoints super useful. I wanted the name of the film. I think it would have affected my analysis because it would bring prior knowledge to the analysis. It could have sparked different hypotheses for me to follow''}
    \item +++- (details view agg) -- \emph{``I don’t really remember the table view in Details. I was visualizing the aggregation and it was good to have for reference.''}
\end{enumerate}


% Awareness
\subsubsection{AWARENESS}

\bpstart{P04}
\begin{enumerate}[nosep]
    \item ++++ (on seeing a white attribute card)``I don't think Release Year should matter too much, hence I am not interacting with it.''
    \item ++++ (on seeing another white attribute card) ``OK, I haven't looked at Content Rating yet...I should take a look at that?''
    \item ++++ (hovered on a white R-rated movies bar and observed the details view) ``There doesn't seem many blue rows means I haven't been focusing on it''
    \item ++++ ``Distribution of my focus on Runtime (blue) is representative of the applied filter.''
\end{enumerate}

\bpstart{P01}
\begin{enumerate}[nosep]
    \item ++++ (motivation for custom target distributions) -- \emph{``I have a younger brother so I want to recommend PG-13 movies only''}
    \item ++++ (interest in the distribution panel) -- ``Let us open up everything in the panel.''
    \item ++++ (positive feedback) -- ``I haven't seen many things like this before...I really liked the UI - very simple to look...really good technique..nice details view''
    \item --++ (blue colorings) - ``very useful..but I learnt about them slightly afterwards...which isn't so bad.'
\end{enumerate}

\bpstart{P02}
\begin{enumerate}[nosep]
    \item ---- (blue colorings) -- ``At one point, I confused (blue) colors with an Encoding''
\end{enumerate}

\bpstart{P03}
\begin{enumerate}[nosep]
    \item ++++ (utility of distribution panel in decision making scenarios) -- \emph{``If I had a specific plan w.r.t. accomplishing the task, e.g. a few attributes, then I would have loved to use this panel a lot more.''}
    \item ++-- (attribute-panel blue colorings) -- \emph{``Actually I forgot, had I remembered, it might have been interesting to not click on the same thing over and over.''}
    \item ---+ (in-situ VIS blue colorings) -- \emph{``coloring was helpful but if it is based on me hovering on a point again and again, it might not be 100\% correct. I analyze the entire visualization with my eyes (focus) and sometimes, out of curiosity, choose to inspect the outliers. In this tool, the latter gets captured as focus instead.''}
\end{enumerate}

\bpstart{P05}
\begin{enumerate}[nosep]
    \item ++++ (distribution panel) -- ``The cool thing here is that I don't need to create visualizations in the VIS panel for each attribute to see their distributions...the Distribution panel is very helpful.''
    \item ++++ (distribution panel) -- ``Participant went through all the attributes once in the Distribution Panel''
    \item ++++ (feature request) ``Can the filter also be applied to the Distribution panel?''
    \item ++++ (on seeing a dark blue attribute panel interaction trace) -- ``I see that I have spent a lot of time on Release Year...so I'll now see something else''.
    \item ++++ (on seeing three red attributes in the distribution panel) -- ``Since I'm not having a targeted approach, I am just thinking aloud + exploring... so now I want to consider what I haven't so far.''
    \item ++++ (on seeing a red Content-Rating attribute) -- ``Seems I didn't interact with R movies enough so this view nudges me towards those (and then applies a filter)''
    \item ++-- (efficacy of blue points) -- ``I am getting drawn to the visited points when I create new visualizations.''
    \item ++-- (feature request) -- ``Can I see which view I interacted this point with?''
    \item ++++ (after some time) -- ``Participant again saw a few red bars and applied filters to try and turn them green.''
    \item ++++ (after some more time) -- ``Participant now tries to balance the white->blue colors in the attribute view''
    \item ++++ (attribute panel interaction traces) -- ``I think this view was very useful for my workflow''
    \item ++-- (red>green distribution panel colors) -- ``The red>green stuff was a bit tough as I didn't know exactly what to do about it. It did not guide me how to correct it.'
    \item ++++ (overall positive feedback) -- ``This is very interesting, there is slight learning curve involved but having help icons, tutorials will solve that; It will be interesting if and how you will integrate this tool into existing tools such as Tableau.''
\end{enumerate}

\bpstart{P06}
\begin{enumerate}[nosep]
    \item ++++ (after seeing the video) -- ``It (the distribution view) gives me a sense if I'm looking at the dataset in an unbiased way.''
    \item ++-- (after creating a new vis) -- ``I didn't expect the blue color on points to stay (since they weren't created here).''
    \item ++++ (details view for agg) -- ``Giving a table for aggregated values is nice''
    \item ++++ (efficacy of distribution panel + motivates need for ACTIVE mitigation strategies) -- ``(participant looked at Genre and saw three interactions with Concert, Documentary, and Westerns genres and said) I should now interact with drama since that is maximum and these are almost nil.... (they began correcting their bias but after a while started being biased towards Drama movies)... (after some more time, they finalize realize their bias towards Drama movies)''
    \item ++-- (attribute panel interaction traces) -- ``My impression - it's also there...but I do get the impression which attributes were not used/focused on''
    \item ++-- (blue points) -- ``I was initially confused but then over use I got used to them and found them useful in tracking visited points''
    \item ---- (details view agg) -- ``Interaction history in details view was not useful''
    \item ++++ (distribution panel) -- ``Helped me a lot''
    \item ++++ (feature request) -- ``Remove older interactions, say only keep the most recent 100/200 of them - people lose attention/trust''
    \item ++-- (awareness vis) -- ``Discrete (bar) charts I can track and channel my focus (by applying filter)...but difficult to discretize and track a continuous attribute.''
    \item ++++ (motivation for ACTIVE mitigation) -- ``I just wish I can directly filter in the awareness widget (especially for continuous attributes)''
    \item ++++ (pinning attributes) -- Useful when there are many attributes
\end{enumerate}

\bpstart{P07}
\begin{enumerate}[nosep]
    \item ++++ (first tryst with distribution panel) -- ``1st click after red-green colors came up was on the red Driveline attribute - participant saw a 100\% focus on All-Wheel-Drive casr and then created a chart with Driveline to inspect''
    \item ++++ (awareness) -- ``Ok so I have focused more on transmission''
    \item ++++ (awareness) -- ``Let's look at production budget, it seems I haven't looked at it at all -- seems important''
    \item ++++ (awareness) -- ``(on looking at the Dramatization bar category in the awareness visualization) See I don't care about Dramatization movies..Who cares?''
    \item ++++ (awareness) -- ``I don't think this (a white Runnng Time bar in the attribute panel) is important to me'
    \item ++++ (awareness) -- ``Geez, I haven't looked at Drama data at all (on looking at the red distribution panel for Genre)'
    \item ++++ (feedback) -- ``I don't really hover on things in e.g., a scatterplot but information shown on hovering a bar chart (the details view agg) was awesome because you showed individual data.'
    \item ++++ (feedback) -- ``I think there are lots of use-cases in journalism (e.g., you have only looked at trending news and this tool can nudge towards other news), social media (e.g., you have only looked at Trump's negative tweets -- what about Biden's?) for this technique. Communicating back to the user how they are doing is something I would use in my tools''
    \item ++++ (distribution panel colors) -- ``The colors were very useful even though I only looked at it for only a bit''
    \item ++++ (feature request) -- ``Consider an interaction (to compute focus) based on proximity and not just an exact mouse hover. Mouse as a proxy for focus has many limitations''
\end{enumerate}

\bpstart{P08}
\begin{enumerate}[nosep]
    \item ++++ (random) -- ``Interacting (with these scatterplot points) and seeing these colors change is fun''
    \item ++++ (active mitigation) -- ``I know that red is bad...does the tool give me a button to apply a reverse filter''
    \item ++++ (awareness) -- ``(after a few interactions) This is so biased - but whatever''
    \item ++++ (interesting feature request) -- Participant created a budget v.s. gross plot and interacted with a few points. Then, considering these interacted points as model/seed movies, they opened the distribution panels to see how they (now in blue) compare to all movies (black) and recommended high-level categories accordingly (e.g., don't make Western and Black Comedy genres as there are no blue bars for them) -- ``The way I'm using this, I want to be able to clear all blue interactions and start a new session with a new set of model movies to compare in the Distribution panel''
    \item ++-- (participant concern) -- ``Now I should be careful to not interact with dots and skew my interaction trace''
    \item ++++ (feedback) -- ``The ability to keep track of your provenance, interaction history is interesting''
    \item ++++ (feedback) -- ``The Distribution panel lets you look at teh false positives if you (compare it to a confusion matrix)''
    \item ++++ (feedback) -- ``I was more interested in the 'red' variables than the green 'ones'''
    \item ---- (details view) -- ``Details view was slightly useful as it is difficult to compare with other datapoints or remember them across views''
    \item ++-- (blue attribute panel colors) -- ``I didn't use the blue attributes panel but now that I see this questions, I would've seen them more''
\end{enumerate}

\bpstart{P13}
\begin{enumerate}[nosep]
    \item ---- (invis blue colorings) -- \emph{``I think highlight the same data point over and over again skews the distribution visualization, which I think could be an issue''.}
    \item --++ (attribute blue color, learning curve) -- \emph{``When an attribute bar in the attributes panel is highlighted, it tells me that I should be able to click on the bar to toggle the color. This is not how it works; I have to click the clear button in the filter panel to remove the filter.''} 
    \item ++++ (feature request, interaction traces on chart type) -- ``The tool didn't tell me how much time I spent on a specific chart, and if it had, I might have wanted to switch up the chart type.''
    \item ++++ (distribution panel) -- ``\emph{I have a good hypothesis -- I’m aware of the panel, it shows me what I spend the most time on. I want to remove the internal bias of what things I think are the most interest. I want the panel to tell me what other things are in the dataset.}''
    \item ++++ (awareness) -- ``\emph{Comedy and Drama are high percentage in the dataset, and I haven’t interacted with them much at all, so it might be worth my time to look at them.}''
    \item ++++ (awareness of categories within data) -- \emph{``Now that I know the categories, let me Filter away some of them... Even though there are a lot of Comedy and Drama movies [by looking at the Distribution panel], when I filter them away, they don’t appear as the highest grossing movies.''}
    \item ++++ (feature request) -- \emph{``I would really love to hover on a value in the categorical filter and have it somehow highlight in the Visualization panel''}
    \item ++++ (attribute blue color) -- \emph{``Looking at how Running Time is not colored at all in the Attributes panel “I haven’t touched Running Time at all”''}
    \item ++-- (awareness, but a limitation of the model) -- \emph{``“I had Release Year on my axis the whole time, but in the attribute panel, the focus was really low, which wasn’t the case for what I cared about.”''}
    \item ---- (colorings in the VIS) -- \emph{``It’s really hard to distinguish the lighter shades of blue on the scatterplot. It’s a lot easier using a bar chart...The coloring as a whole doesn’t help me make decisions about my data''}
    \item ++++ (red-gray-green vis in Distribution panel) -- \emph{``I found this really really useful. This gave me a really easy way to show me what my focus was. This was an improved version of the coloring in the visualization.''}
    \item ++++ (vis in Distribution panel) -- \emph{``I think having “new data” vs “same data” distinction here might be helpful. Showing me when I hover on a new movie vs hovering multiple times in the same movie. The bar could get really high if I keep looking at the same data point.''}
    \item ++-- (personality, distraction) -- \emph{``I never had a need to bookmark. I’m just not going to look at the panel until after I’m done with my analysis. While I’m doing my analysis, the bars will be moving, and that’s distracting''}
\end{enumerate}

\bpstart{P15}
\begin{enumerate}[nosep]
    \item ++++ (general feedback) -- \emph{``Tool was pretty intuitive to navigate around
    ''}
    \item ---- (mousehover shouldn't be a proxy for focus) -- \emph{When you hover over a point the color is recorded, even if I wasn’t interested in the point. That was inaccurate for my focus. Because of this, I tuned out the coloring for datapoints -- which were lighter blue and which were darker blue.}
    \item ---- (red-gray-green didn't help) -- \emph{``I also didn’t pay attention to the green versus red coloring. I was focused on answering my own questions, and I didn’t use the color to help me make any decisions. They weren’t as helpful to me.''}
    \item ++++ (details view) -- \emph{``“Details view would be much more useful for multivariate hypotheses, which I did not have!''}
    \item ++-- (distribution panel) -- \emph{``The Distribution panel was an afterthought. I didn’t know how to use it in the context of  what I was doing. It was also tucked away on the right side of the screen, and this fell out of focus for me. I was really focused on the left and middle parts of the screen. If I had more time to do this, I would have probably eventually looked into the Distribution panel.''}
\end{enumerate}

\bpstart{P22}
\begin{enumerate}[nosep]
    \item ++++ (derived insight from distrubution panel) -- \emph{``I noticed that Adventure is representative of most values in Rotten Tomatoes Rating and IMDB Rating...This is because I mostly interacted with just Adventure movies and that caused those attributes [in the Distribution] to be colored green”''}
    \item ++++ (awareness) -- \emph{``“Now I want to look at attributes that I haven’t been paying attention to...To do this, they looked at the coloring of the Distribution panel bars rather than the Attributes panel!''}
    \item ++++ (curiosity) -- \emph{``User appeared to hover multiple times on the same bar to see how a pinned attribute in the Distribution panel changed (both visualization and color)''}
    \item ++++ (awareness) -- \emph{``Noticed that Running Time is really white at this point in the Attributes panel -- Ok, now I’m going to interact with Running Time''}
    \item ---- (details view agg) -- \emph{``Having the Details table colored was confusing... I didn’t know what that meant.''}
    \item ++-- (curiosity) -- \emph{``“One thing that wasn’t clear was how the coloring the Visualization panel was being applied. I think it was somewhat intuitive… but I generally wanted an explanation of how it worked to feel better about it. During transition between encodings, I wasn’t sure how the coloring was updating''}
    \item ++++ (distribution panel) -- \emph{``“The Distribution panel was a GREATTTTT idea, I loved it so much!”''}
\end{enumerate}

==> src/tables/vis-matrix.tex <==
\begin{tabular}{lll}
    \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Attributes}\\\small{(X,Y)}\end{tabular}} &
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Aggregation}\\\small{(Agg)}\end{tabular}} &
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Visualizations}\\\small{(Chart Type)}\end{tabular}} \\ \\

    \hline

    \multirow{1}{*}{N, T, \{Q\} x \{N, T, Q\}} & 
    \multirow{1}{*}{-} &
    \multirow{1}{*}{Scatter Plot} \\

    \multirow{1}{*}{Q x \{N, T\}} & 
    \multirow{1}{*}{-} &
    \multirow{1}{*}{Strip Plot} \\

    \multirow{2}{*}{N, T, Q x \{Q\}} & 
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Count, \{Average,\\ Sum, Min, Max\}\end{tabular}} &
    \multirow{2}{*}{Bar Chart} \\ \\

    \multirow{2}{*}{T x \{Q\}} & 
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Count, \{Average,\\Sum, Min, Max\}\end{tabular}} &
    \multirow{2}{*}{Line Chart} \\ \\ 
    
    \hline
\end{tabular}%
